Assessing Spatial Disparities: A Bayesian Linear Regression Approach

Epidemiological investigations of regionally aggregated spatial data often involve detecting spatial health disparities among neighboring regions on a map of disease mortality or incidence rates. Analyzing such data introduces spatial dependence among health outcomes and seeks to report statistically significant spatial disparities by delineating boundaries that separate neighboring regions with disparate health outcomes. However, there are statistical challenges to appropriately define what constitutes a spatial disparity and to construct robust probabilistic inferences for spatial disparities. We enrich the familiar Bayesian linear regression framework to introduce spatial autoregression and offer model-based detection of spatial disparities. We derive exploitable analytical tractability that considerably accelerates computation. Simulation experiments conducted on a county map of the entire United States demonstrate the effectiveness of our method, and we apply our method to a data set from the Institute of Health Metrics and Evaluation (IHME) on age-standardized US county-level estimates of lung cancer mortality rates.

==> figures/BYM2_sim/US_gibbs/epsilon_sensitivity_table.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Sat Nov  1 12:27:13 2025
\begin{table}[ht]
\centering
\begin{tabular}{ccccccc}
  \hline
$\epsilon$ & $t_{\star}$ & Detected Boundaries & True Boundaries & Sensitivity & Specificity & Accuracy \\ 
  \hline
0.562 & 0.811 & 6070 & 7609 & 0.742 & 0.721 & 0.739 \\ 
  1.124 & 0.832 & 4212 & 6188 & 0.638 & 0.909 & 0.725 \\ 
  1.685 & 0.856 & 2838 & 4841 & 0.553 & 0.962 & 0.745 \\ 
  2.247 & 0.874 & 1756 & 3679 & 0.454 & 0.985 & 0.771 \\ 
  2.809 & 0.886 &  983 & 2674 & 0.352 & 0.994 & 0.806 \\ 
   \hline
\end{tabular}
\caption{Cutoff probabilities, number of detected/true difference boundaries, and
                     classification performance with Bayesian FDR tolerance $\delta = 0.05$
                     across different values of difference threshold $\epsilon$.} 
\label{tab:epsilon_sensitivity}
\end{table}


==> figures/lung_RDA/US_data/params_summary.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Sat Nov  1 05:57:17 2025
{\color{blue}
\begin{table}[ht]
\centering

\begin{tabular}{cccc}
  \hline
Parameter & Description & Posterior Mean & 95\% Credible Interval \\ 
  \hline
$\beta_0$ & Intercept & 9.56 & (4.828, 14.223) \\ 
  $\beta_1$ & Smoking prevalence & 1.90 & (1.754, 2.052) \\ 
  $\beta_2$ & Unemployment Percentile & 1.85 & (-0.473, 4.174) \\ 
  $\beta_3$ & SVI Percentile & 5.70 & (2.755, 8.68) \\ 
  $\beta_4$ & Physically Inactive (\%) & 0.35 & (0.202, 0.49) \\ 
  $\beta_5$ & Uninsured (\%) & -0.60 & (-0.746, -0.451) \\ 
  $\beta_6$ & Diabetes Prevalence (\%) & 0.18 & (-0.137, 0.506) \\ 
  $\beta_7$ & Obesity Prevalence (\%) & 0.06 & (-0.08, 0.2) \\ 
  $\sigma^2$ & Total variance & 108.25 & (95.927, 123.349) \\ 
  $\rho$ & Spatial proportion of variance & 0.78 & (0.692, 0.861) \\ 
   \hline
\end{tabular}
\caption{Posterior summaries of non-spatial effect parameters in analysis of US county-level lung cancer mortality rates.}
\label{tab:RDA_post_summaries}
\end{table}
}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
